Revisiting the Impact of Dust Production from Carbon-Rich Wolf-Rayet Binaries

We present a dust spectral energy distribution (SED) and binary stellar population analysis revisiting the dust production rates (DPRs) in the winds of carbon-rich Wolf-Rayet (WC) binaries and their impact on galactic dust budgets. DustEM SED models of 19 Galactic WC ``dustars" reveal DPRs of $\dot{M}_d\sim10^{-10}-10^{-6}$ M$_\odot$ yr$^{-1}$ and carbon dust condensation fractions, $\chi_C$, between $0.002 - 40\%$. A large ($0.1 - 1.0$ $\mu$m) dust grain size composition is favored for efficient dustars where $\chi_C\gtrsim1\%$. Results for dustars with known orbital periods verify a power-law relation between $\chi_C$, orbital period, WC mass-loss rate, and wind velocity consistent with predictions from theoretical models of dust formation in colliding-wind binaries. We incorporated dust production into Binary Population and Spectral Synthesis (BPASS) models to analyze dust production rates from WC dustars, asymptotic giant branch stars (AGBs), red supergiants (RSGs), and core-collapse supernovae (SNe). BPASS models assuming constant star formation (SF) and a co-eval $10^6$ M$_\odot$ stellar population were performed at low, Large Magellanic Cloud (LMC)-like, and solar metallicities (Z = 0.001, 0.008, and 0.020). Both constant SF and co-eval models show that SNe are net dust destroyers at all metallicities. Constant SF models at LMC-like metallicities show that AGB stars slightly outproduce WC binaries and RSGs by factors of $2-3$, whereas at solar metallicites WC binaries are the dominant source of dust for $\sim60$ Myr until the onset of AGBs, which match the dust input of WC binaries. Co-eval population models show that for "bursty" SF, AGB stars dominate dust production at late times ($t\gtrsim 70$ Myr).

==> BPASS_SMC.tex <==
\begin{deluxetable}{lll}
\tablecaption{BPASS SMC Dust Model Table}
\tablewidth{10pt}
\tablehead{ & BPASS ($t = 12.6$ Gyr) & From Obs. }
\startdata
	N$_{AGB}$ & 3500 & 3516 \\ 
	N$_{RSG}$ & 1506 & 1410 \\ 
	N$_{WC}$ & 63 & - \\ 
	R$_{SN}$ (yr$^{-1}$) & $9.9\times10^{-3}$ & $(1.11\pm0.27)\times10^{-3}$ \\ 
	$\dot{M}_{AGB}$(M$_\odot$ yr$^{-1}$) & $6.4\times10^{-7}$ [$1.4\times10^{-10}$] & $1.3\times10^{-6}$ [$3.7\times10^{-10}$] \\ %need to check Srinivasan AGB numbers.. mean seems off
	$\dot{M}_{RSG}$ (M$_\odot$ yr$^{-1}$) & $2.4\times10^{-7}$ [$8.0\times10^{-11}$] & $4.6\times10^{-8}$ [$3.3\times10^{-11}$] \\ 
	$\dot{M}_{WC}$ (M$_\odot$ yr$^{-1}$) & $4.3\times10^{-5}$ [$6.4\times10^{-7}$] & - \\ 
	$\dot{M}_{SN}$ (M$_\odot$ yr$^{-1}$, M$_\odot$) & $1.1\times10^{-3}$ [$0.11$] & $3.9\times10^{-4}$ [$\sim0.4$] \\ 
	Log($t_{0,AGB}$) & 8.5 & - \\ 
	Log($t_{0,RSG}$) & 6.3 & - \\ 
	Log($t_{0,WC}$) & 6.3 & - \\ 
	Log($t_{0,SN}$) & 6.6 & - \\ 
\enddata
\tablecomments{\citep{Srinivasan2016,Temim2015} X-ray, IR, and derived dust properties of the 4 ``red" mid-IR ULX counterpart candidates including the ULX name, X-ray (2 - 10 keV) luminosity, dust temperature, IR luminosity, total dust mass, dust equilibrium temperature radius, dust sublimation radius. A heating source with a luminosity equivalent to the IR luminosity and a 20000 K photosphere ($\left<Q\right>_{*}/ \left<Q\right>_{IR} = 30$) is adopted for equilibrium radius calculation. For the R$_\mathrm{sub}$ calculation, a heating source with a luminosity equivalent to $L_X$ value is adopted and $\left<Q\right>_{X}/ \left<Q\right>_{IR} = 1$.}
\label{tab:BPASSSMCTab}
\end{deluxetable}


